Interpretable Image Classification via Non-parametric Part Prototype Learning

Classifying images with an interpretable decision-making process is a long-standing problem in computer vision. In recent years, Prototypical Part Networks has gained traction as an approach for self-explainable neural networks, due to their ability to mimic human visual reasoning by providing explanations based on prototypical object parts. However, the quality of the explanations generated by these methods leaves room for improvement, as the prototypes usually focus on repetitive and redundant concepts. Leveraging recent advances in prototype learning, we present a framework for part-based interpretable image classification that learns a set of semantically distinctive object parts for each class, and provides diverse and comprehensive explanations. The core of our method is to learn the part-prototypes in a non-parametric fashion, through clustering deep features extracted from foundation vision models that encode robust semantic information. To quantitatively evaluate the quality of explanations provided by ProtoPNets, we introduce Distinctiveness Score and Comprehensiveness Score. Through evaluation on CUB-200-2011, Stanford Cars and Stanford Dogs datasets, we show that our framework compares favourably against existing ProtoPNets while achieving better interpretability. Code is available at: https://github.com/zijizhu/proto-non-param.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/X_rebut.tex <==
\clearpage
\setcounter{page}{1}

\twocolumn[\centering\section*{Interpretable Image Classification via Non-parametric Part Prototype Learning (Rebuttal)}]

\textbf{R1-1 Classification Accuracy.} Our work primarily focuses on enhancing the interpretability of classification models rather than aiming to improve accuracy. Previous studies have highlighted the inherent tradeoff between accuracy and interpretability \cite{espinosa_zarlenga_concept_2022,chen_this_2019}. Our method preserves high accuracy while offering interpretability with desirable properties, such as distinctiveness and comprehensiveness, which have been largely overlooked in prior works.

\textbf{R1-2 Consistency Scores.} As shown in Table \ref{tab:main-protopnets-results} in the paper, although our method does not always achieve highest consistency scores, they are comparable to \cite{huang_evaluation_2023}, which employs a dedicated module for improving consistency. For a simpler and more computationally efficient architecture, our method was not trained with such module, and the consistency scores were just $2.4\%$ lower than \cite{huang_evaluation_2023} when $K=5$, and $3.9\%$ higher when averaged over all experiments. Overall, our method achieves better performance on a wider range of interpretability criteria with decent consistency.

\textbf{R1-3 Experiments in Table 1 and Table 2.} To show the generalization ability of our method, we have presented experimental results against other ProtoPNets on Stanford Cars \cite{krause_3d_2013} and Stanford Dogs \cite{dataset2011novel} in Table \ref{tab:supp-cars-results} and Table \ref{tab:supp-dogs-results} of supplementary material following previous works. Regarding Table \ref{tab:concept-learning-results}, our method and \cite{huang_concept_2024} are the only methods that can accurately localize concepts under concept learning setting. Other CBM models rely on CAM-based methods when localized explanation is needed, which has been shown to provide unfaithful explanation \cite{huang_concept_2024}. For further comparison, we have included more results of CBMs for concept learning in Table \ref{tab:rebuttal-cbm-results} here in this rebuttal.

\textbf{R2-1 Change of the backbone to ViT.} The ViT backbone does improve accuracy of previous methods compared to CNNs, ranging from $5\%$ to $10\%$. However, explanations generated using existing techniques applied to ViT backbones are often inconsistent and fail to satisfy interpretability metrics, as shown in Table \ref{tab:main-protopnets-results} (in the paper) and Figure \ref{fig:distinctiveness-comprehensiveness}. Note that DINOv2 ViT-B achieves $91.3\%$ on CUB-200-2011 via linear probing on cls tokens, so applying original ProtoPNet with ViT naively also results in around $3\%$ drop in accuracy. This demonstrates the tradeoff between interpretability and performance. In contrast, our method effectively leverages the deep features of ViTs to provide consistently interpretable explanations while maintaining minimal performance degradation with an accuracy of $90.82\%$.

\textbf{R2-2 Foreground Extraction Module.} It is a component that selects foreground ViT patch tokens so that the prototype updates are computed from foreground tokens that contain meaningful information about the object. This can be implemented by various off-the-shelf methods which do not need training and can be applied on deep ViT features. We have omitted it in the main paper since it is not the focus of our method, however the technical details and the ablation study of different extraction methods are provided in Section \ref{sec:supp-results} and Table \ref{tab:ablation-fg-extraction} of supplementary material.

\textbf{R2-3 Equation \ref{eq:8}.} The model performs foreground extraction in both prototype learning and fine-tuning stages right after the tokens are extracted from frozen backbones, thus $\mathbf{f}^c_i$ in Eq. \ref{eq:8} represent only foreground tokens in an input image belonging to class $c$. The background patch tokens are not involved in the computation of this loss.

\textbf{R3-1 Compared methods.} We included a number of comparisons against EvalProtoPNet \cite{huang_evaluation_2023}, the best performing Interpretable classifier on CUB-200-2011 with a higher accuracy than PIP-Net and ST-ProtoPNet. For further comparison, we now show the result of PIP-Net and ST-ProtoPNet evaluated with DINOv2 ViT-B on CUB-200-2011 in Table \ref{tab:rebuttal-results} here in this rebuttal (PIP-Net has a different style of visual explanations so only accuracy is evaluated).

\setcounter{table}{0}

\begin{table}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
      \begin{tabular}{lccccc}
        \toprule
        & Con. & Sta. & Dis. & Comp. & Acc. \\
        \midrule
        PIP-Net & N/A & N/A & N/A & N/A & 89.91 \\
        ST-ProtoPNet & 47.18 & 66.10 & 70.93 & 83.28 & 89.79 \\
        Ours & 66.40 & 82.97 & 94.45 & 93.49 & 90.82 \\
        \bottomrule
        \vspace{-1.9em}
      \end{tabular}
    }
    \caption{Interpretability (\%) and accuracy (\%) of ST-ProtoPNet and PIP-Net evaluated with DINOv2 ViT-B on CUB-200-2011.}
    \label{tab:rebuttal-results}
    \vspace{-1em}
  \end{table}

  \begin{table}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
      \begin{tabular}{lcccc}
        \toprule
        & Vanilla CBM \cite{koh_concept_2020} & h-CBM & CEM \cite{espinosa_zarlenga_concept_2022} & Ours \\
        \midrule
        Loc. & 15.63 & 11.62 & 20.10 & 47.04 \\
        Acc. & 90.06 & 88.24 & 86.87 & 88.18 \\
        \bottomrule
        \vspace{-2em}
      \end{tabular}
    }
    \caption{Concept learning performance (\%) of various CBMs evaluated with DINOv2 ViT-B and CAM. h-CBM is vanilla CBM with a residual connection to the output layer.}
    \label{tab:rebuttal-cbm-results}
    \vspace{-2em}
  \end{table}

\textbf{R3-2.1 Differences between our method and \cite{zhou_rethinking_2022}.} For prototype learning, the prototypes in our method are learned in a dedicated training stage without fine-tuning the backbone, while \cite{zhou_rethinking_2022} trains the backbone and the prototypes at the same time. In addition, the prototypes serve as final classification weights in \cite{zhou_rethinking_2022}, whereas in our framework, the prototypes are used to produce interpretable activation maps. Regarding the Patch-Prototype Optimization loss, note that in our method $\mathcal{P}^{-}$ is the set of prototypes belonging to the same class as the one assigned to the patch, which is different to $\mathcal{P}^{-}$ in \cite{zhou_rethinking_2022} that includes prototypes from all classes. Hence our loss function only separates each patch from other prototypes from the same class, which is significantly different to the one in  \cite{zhou_rethinking_2022}.

\textbf{R3-2.2 Novelty.} While the mathematics behind prototype learning is similar to \cite{zhou_rethinking_2022}, our method is the first to explore its use in interpretable classification. To this end, we have made significant changes to the overall architecture and introduced novel two-stage training strategy and loss function, so that prototype learning can be well adapted.

We thank reviewers for pointing out the typos in minor weaknesses, we will fix them accordingly.

==> sec/figures/supp_reasoning_visualization.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{C}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{1cm}}
\newcommand{\myimg}[1]{\raisebox{-.5\height}{\includegraphics[width=0.18\columnwidth]{#1}}}
\newcommand{\myimgsmall}[1]{\raisebox{-0.0\height}{\includegraphics[scale=0.15]{#1}}}
\newcommand{\myimgmedium}[1]{\raisebox{-0.5\height}{\includegraphics[scale=0.3]{#1}}}
\renewcommand{\arraystretch}{0.25}

\begin{table*}
  \centering
  \begin{tabular}{cc}
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{American Pipit ?}}} & \myimgsmall{sec/figures/American_Pipit_0119_99622/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimg{sec/figures/American_Pipit_0119_99622/part0.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/source0.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/activations0.jpg} & 2.92 \\
      \\
      \myimg{sec/figures/American_Pipit_0119_99622/part1.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/source1.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/activations1.jpg} & 2.33 \\
      \\
      \myimg{sec/figures/American_Pipit_0119_99622/part2.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/source2.jpg} & \myimg{sec/figures/American_Pipit_0119_99622/activations2.jpg} & 2.71 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    } &
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{Ringed Kingfisher ?}}} & \myimgsmall{sec/figures/Ringed_Kingfisher_0005_73086/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimg{sec/figures/Ringed_Kingfisher_0005_73086/part0.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/source0.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/activations0.jpg} & 3.05 \\
      \\
      \myimg{sec/figures/Ringed_Kingfisher_0005_73086/part1.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/source1.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/activations1.jpg} & 2.43 \\
      \\
      \myimg{sec/figures/Ringed_Kingfisher_0005_73086/part2.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/source2.jpg} & \myimg{sec/figures/Ringed_Kingfisher_0005_73086/activations2.jpg} & 2.73 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    } \\
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{Western Grebe ?}}} & \myimgsmall{sec/figures/Western_Grebe_0102_36116/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimgmedium{sec/figures/Western_Grebe_0102_36116/part4.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/source4.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/activations4.jpg} & 3.09 \\
      \\
      \myimgmedium{sec/figures/Western_Grebe_0102_36116/part1.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/source1.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/activations1.jpg} & 2.82 \\
      \\
      \myimgmedium{sec/figures/Western_Grebe_0102_36116/part2.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/source2.jpg} & \myimg{sec/figures/Western_Grebe_0102_36116/activations2.jpg} & 2.52 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    } &
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{Clark Nutcracker ?}}} & \myimgsmall{sec/figures/Clark_Nutcracker_0102_85089/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimgmedium{sec/figures/Clark_Nutcracker_0102_85089/part4.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/source4.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/activations4.jpg} & 2.93 \\
      \\
      \myimgmedium{sec/figures/Clark_Nutcracker_0102_85089/part3.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/source3.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/activations3.jpg} & 2.99 \\
      \\
      \myimgmedium{sec/figures/Clark_Nutcracker_0102_85089/part0.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/source0.jpg} & \myimg{sec/figures/Clark_Nutcracker_0102_85089/activations0.jpg} & 2.82 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    } \\
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{Great Grey Shrike ?}}} & \myimgsmall{sec/figures/Great_Grey_Shrike_0005_797055/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimgmedium{sec/figures/Great_Grey_Shrike_0005_797055/part4.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/source4.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/activations4.jpg} & 2.99 \\
      \\
      \myimgmedium{sec/figures/Great_Grey_Shrike_0005_797055/part0.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/source0.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/activations0.jpg} & 3.02 \\
      \\
      \myimgmedium{sec/figures/Great_Grey_Shrike_0005_797055/part2.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/source2.jpg} & \myimg{sec/figures/Great_Grey_Shrike_0005_797055/activations2.jpg} & 3.28 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    } &
    \resizebox{\columnwidth}{!}{
    \begin{tabularx}{\columnwidth}{Y Y Y C}
      \multicolumn{3}{l}{\makecell{\textbf{Why is this image classified as a} \\ \textbf{Yellow Warbler ?}}} & \myimgsmall{sec/figures/Yellow_Warbler_0071_176655/input.jpg} \\
      \\
      \toprule
      \textbf{Prototypical Part} & \textbf{Source Image} & \textbf{Activation Map} & \textbf{Score} \\
      \midrule
      \myimgmedium{sec/figures/Yellow_Warbler_0071_176655/part2.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/source2.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/activations2.jpg} & 2.88 \\
      \\
      \myimgmedium{sec/figures/Yellow_Warbler_0071_176655/part1.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/source1.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/activations1.jpg} & 2.73 \\
      \\
      \myimgmedium{sec/figures/Yellow_Warbler_0071_176655/part4.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/source4.jpg} & \myimg{sec/figures/Yellow_Warbler_0071_176655/activations4.jpg} & 3.26 \\
      \\
      $\dots$ & $\dots$ & $\dots$ & $\dots$ \\
    \end{tabularx}
    }
  \end{tabular}
  \caption{Visualization of the typical visual reasoning process of our framework on CUB-200-2011 dataset.}
  \label{tab:supp-reasoning}
\end{table*}


==> sec/supp_algo.tex <==
\begin{algorithm}
\caption{Prototype Learning and Backbone Fine-tuning}
\label{alg:training}
\begin{algorithmic}[1]
  \Require Training set $\mathcal{X}$, $nEpochs$, ViT backbone $\mathcal{F}$
\State Initialize prototypes $\mathbf{P}$ and modulation vector $w$ with $\mathbf{P} \sim \mathcal{N}(0.0, 0.02)$ and $w^c_k=0.2$
\For{$t \in \{1, \dots, nEpochs\}$}
    \State Randomly split $\mathcal{X}$ into mini-batches
    \For{$(\mathbf{X}, \mathbf{y}) \in \{\mathcal{X}_1, \dots\}$}
        \State $\mathbf{f} = \text{reshape}(\mathcal{F}(\mathbf{X})) \in \mathbb{R}^{Bhw \times D}$
        \State $\mathcal{M} = \phi(\mathbf{f}, \mathbf{X}) \in \{0, 1\}^{Bhw}$
        \State $\mathbf{S} = \text{reshape}(\text{Sim}(\mathbf{f}, \mathbf{P})) \in \mathbb{R}^{Bhw \times N \times K}$
        \For{$c \in \text{unique}(\mathbf{y})$}
          \State Get $\mathbf{S}^c$ and $\mathbf{f}^c$ by indexing $\mathbf{S}$, $\mathbf{f}$ with $\mathcal{M}$, $\mathbf{y}$
          \State $\mathbf{A}^{c,*} = \text{sinkhorn\_knopp}(\mathbf{S}^c)$
          \If{\textit{first training stage}}
            \State $\mathbf{P}^c \leftarrow \beta \mathbf{P}^c + (1 - \beta) (\mathbf{A}^{c,*})^\top\mathbf{f}^c$
          \EndIf
        \EndFor
        \State $g = \text{MaxPool}(\text{reshape}(\mathbf{S})) \in \mathbb{R}^{N \times K}$
        \State $\text{logits} = \text{compute\_logits}(g, w) \in \mathbb{R}^N$
        \If{\textit{second training stage}}
          \State Compute loss $\mathcal{L}_{xe}(\text{logits}, \mathbf{y})$
          \State Compute loss $\mathcal{L}_{PPC}(\mathbf{S}, \mathbf{A})$
          \State Minimize loss by updating $\mathcal{F}$
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


==> sec/supp_compre_algo.tex <==
\begin{algorithm}[t]
  \caption{Python-like pseudo-code of Comprehensiveness Score calculation.}
  \label{alg:compre}
  \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
  \lstset{
    backgroundcolor=\color{white},
    basicstyle=\fontsize{6pt}{6pt}\ttfamily\selectfont,
    columns=fullflexible,
    breaklines=true,
    captionpos=b,
    commentstyle=\fontsize{6pt}{6pt}\color{codeblue},
    keywordstyle=\fontsize{6pt}{6pt},
  }
\begin{lstlisting}[language=python]

def normalize(activations):
    activations = activations.unsqueeze(0)
    max_values = F.adaptive_max_pool2d(activations, (1, 1))
    min_values = -F.adaptive_max_pool2d(-activations, (1, 1))
    return (activations - min_values) / (max_values - min_values)

def calculate_iou(mask1, mask2, eps=1e-6):
    intersection = torch.sum(mask1 & mask2)
    union = torch.sum(mask1 | mask2)
    IoU = intersection / (union + eps)
    return IoU
		
def evaluate_comprehensiveness(model, test_dataset, threshold):
    all_IoUs = []
    for (image, ground_truth_foreground_map) in test_dataset:
        activations = model.get_activation(images) # shape: K, H, W
        activations = normalize(activations)
        activations_union = (activations >= threshold).sum(dim=0)
        IoU = calculate_IoU(
            activations_union,
            ground_truth_foreground_map
        )
        all_IoUs.append(IoU)
    return mean(all_IoUs)
\end{lstlisting}
\end{algorithm}


==> sec/supp_distinc_algo.tex <==
\begin{algorithm}[t]
  \caption{Python-like pseudo-code of Distinctiveness Score calculation.}
  \label{alg:distinctiveness}
  \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
  \lstset{
    backgroundcolor=\color{white},
    basicstyle=\fontsize{6pt}{6pt}\ttfamily\selectfont,
    columns=fullflexible,
    breaklines=true,
    captionpos=b,
    commentstyle=\fontsize{6pt}{6pt}\color{codeblue},
    keywordstyle=\fontsize{6pt}{6pt},
  }
\begin{lstlisting}[language=python]
def evaluate_distinctiveness(model, test_dataset, bbox_size):
    all_O_x = []
    for image in test_dataset:
        activations = model.get_activation(images) # shape: K, H, W
        sample_IoUs = []
        for i in range(K):
            for j in range(K):
                activation_i_max_coord = max_coord(activations[i])
                activation_j_max_coord = max_coord(activations[j])
                bbox_i = get_bbox(activation_i_max_coord)
                bbox_j = get_bbox(activation_j_max_coord)
                IoU = compute_box_IoU(bbox_i, bbox_j)
                sample_IoUs.append(IoU)
        O_x = mean(sample_IoUs)
        all_O_x.append(O_x)
    return 1 - mean(all_O_x)
\end{lstlisting}
\end{algorithm}


==> sec/tables/supp_cars_results.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}
  \centering
  \resizebox{0.95\columnwidth}{!}{
  \begin{tabularx}{\columnwidth}{c|Y|Y}
    \toprule
      \textbf{Methods} & \textbf{ViT-B} & \textbf{ViT-S} \\
      \midrule
      ProtoPNet (K=3) & 86.47 & 78.16 \\
      ProtoPNet (K=5) & 86.75 & 79.51 \\
      \hline
      TesNet (K=3) & 87.33 & 80.97 \\
      TesNet (K=5) & 87.15 & 82.55 \\
      \hline
      EvalProtoPNet & 91.20 & 83.40 \\
      EvalProtoPNet & 91.46 & \textbf{87.09} \\
      \hline
      Ours (K=3) & 91.29 & 85.52 \\
      Ours (K=5) & \textbf{93.63} & 86.10 \\
      \bottomrule
    \end{tabularx}
  }
  \caption{Classification results on Stanford Cars dataset. All methods are trained with DINOv2. Best results are in bold.}
  \label{tab:supp-cars-results}
\end{table}


==> sec/tables/supp_dogs_results.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}
  \centering
  \resizebox{0.95\columnwidth}{!}{
  \begin{tabularx}{\columnwidth}{c|Y|Y}
    \toprule
      \textbf{Methods} & \textbf{ViT-B} & \textbf{ViT-S} \\
      \midrule
      ProtoPNet (K=3) & 84.11 & 79.25 \\
      ProtoPNet (K=5) & 84.90 & 79.28 \\
      \hline
      TesNet (K=3) & 85.16 & 82.14 \\
      TesNet (K=5) & 87.44 & 82.01 \\
      \hline
      EvalProtoPNet & 87.88 & 83.68 \\
      EvalProtoPNet & 88.08 & 83.80 \\
      \hline
      Ours (K=3) & 87.05 & 83.11 \\
      Ours (K=5) & \textbf{88.59} & \textbf{83.93} \\
      \bottomrule
    \end{tabularx}
  }
  \caption{Classification results on Stanford Dogs dataset. All methods are trained with DINOv2. Best results are in bold.}
  \label{tab:supp-dogs-results}
\end{table}


==> sec/tables/supp_fg_extraction_ablation.tex <==
\begin{table}[b]
  \centering
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
      \toprule
      & Con. & Sta. & Dis. & Class. \\
      \hline
      No foreground extraction & 29.67 & 82.85 & 94.17 & 88.42 \\
      PaPr w/ resnet18 & 51.01 & 82.33 & 97.23 & 88.76 \\
      Attention Rollout & 61.90 & 79.97 & 92.77 & 90.75 \\
      First Principal Component & \textbf{66.40} & \textbf{82.97} & \textbf{94.45} & \textbf{90.82} \\
      \bottomrule
    \end{tabular}
  }
  \caption{The effect of various off-the-shelf ViT foreground patch extraction methods on the performance of our framework.}
  \label{tab:ablation-fg-extraction}
\end{table}

